PipelineProfiler: A Visual Analytics Tool for the Exploration of AutoML Pipelines

In recent years, a wide variety of automated machine learning (AutoML) methods have been proposed to search and generate end-to-end learning pipelines. While these techniques facilitate the creation of models for real-world applications, given their black-box nature, the complexity of the underlying algorithms, and the large number of pipelines they derive, it is difficult for their developers to debug these systems. It is also challenging for machine learning experts to select an AutoML system that is well suited for a given problem or class of problems. In this paper, we present the PipelineProfiler, an interactive visualization tool that allows the exploration and comparison of the solution space of machine learning (ML) pipelines produced by AutoML systems. PipelineProfiler is integrated with Jupyter Notebook and can be used together with common data science tools to enable a rich set of analyses of the ML pipelines and provide insights about the algorithms that generated them. We demonstrate the utility of our tool through several use cases where PipelineProfiler is used to better understand and improve a real-world AutoML system. Furthermore, we validate our approach by presenting a detailed analysis of a think-aloud experiment with six data scientists who develop and evaluate AutoML tools.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> text/Interview_analysis_tmp.tex <==
\subsubsection{Data Scientist Insights}

\paragraph{Data pre-processing: } Before they started the investigation, two developers had to remove outliers from their datasets. D1 and D3 selected datasets with a Mean Squared Error evaluation metric, which is unbounded in the positive real numbers. The two selected datasets, Auto MPG \cite{dua2017uci} and Sunspots \cite{sidc2019sunspots}, had pipelines with error metrics above $100,000.0$, which made the scales difficult to read. In both datasets, the data scientists looked at the Primitive Contribution View and noted that a problem with the ``SGD'' primitive was likely responsible for these high errors.  They used \systemname subset menu to remove these pipelines from the analysis.

\paragraph{Performance Investigation}: Most participants started the analysis by looking at the performance of the pipelines. All developers were interested in how their systems compared against the others. Evaluators, on the other hand, focused on the distribution of scores of all systems. For example, the first comparison E1 did was using the pipeline scores. She grouped pipelines by source and noticed the difference in scores among the top pipelines from each AutoML system. The top two AutoML systems had pipelines with F1 Scores of 0.78 and 0.70, which she mentioned were very close. The other systems produced pipelines with much lower scores, below 0.25.

\paragraph{Primitive Comparison: } participants were very interested in comparing pipelines produced multiple systems. In particular, developers spent a considerable amount of time comparing pipelines from their systems against pipelines from the other AutoML tools. For example, D4 inspected a classification dataset and  found that while a gradient boosting algorithm was used in the top scoring pipelines, his system was using decision trees. The Primitive Contribution view confirmed his hypothesis that the use of gradient boosting  was indeed  correlated with high scores. He mentioned that he could use this insight to drop and replace primitives in his AutoML search space. D1, D2 and D3 had similar findings in their pipeline investigations.  Evaluators compared primitive usage for a different reason: they wanted to make sure AutoML systems were exploring the search space and the primitives available to their systems. For example, E1 noticed that the best AutoML system used a single classifier type on its pipelines, as opposed to other systems that had more diverse solutions. E2 did a similar analysis on his dataset.


\paragraph{Hyperparameter Search Strategy: } D1 noticed that the top five pipelines belonged to the same AutoML system, and were nearly identical. She explored the hyperparameters of these pipelines using the  one-hot-encoded hyperparameter view, and found that although they had the same graph structure, they were using different hyperparameters on the ``Gradient Boosting'' primitive. She compared this strategy with another system which did not tune many hyperparameters, and concluded that tuning parameters was beneficial for this problem.

\paragraph{Primitive correctness:} Data scientists also used \systemname to check if primitives were being used correctly. A common finding was the unnecessary use of primitives. For example, D2 found that pipelines containing ``Cast to Type''  resulted in lower F1 scores. He inspected the hyperparameters of this primitive and noted that string features were being converted to float values (hashes). He concluded that string hashes were bad features for this classification problem, and the ``Cast to Type'' primitive should be removed from those pipelines. Similar findings occurred with ``One Hot Encoder'' and pipelines with no categorical features (D3, E1, E2), and ``Imputer'' used on datasets with no missing data (D4, E1). E2 also found incorrect hyperparameter settings, such as the use of ``warm-start=true'' in a ``Random Forest'' primitive.

\paragraph{Running time investigation:} D4 checked the running times of the pipelines. In particular, he was interested in whether the best pipelines took longer to run. First he sorted the pipelines by score. Then, he switched the displayed metric to ``Time'' and noticed that, contrary to his original hypothesis, the best pipelines were also the fastest. He looked at the Primitive Contribution View in order to find what primitives were responsible for the longer running times, and identified that the ``General Relational Dataset'' primitive was most likely the culprit. He concluded that if he removed this primitive, he would get a faster pipeline. 


==> text/sencond_interview_bulletpoints.tex <==

\subsubsection{Developers Interview}

Diego: (D2)
\begin{itemize}
    \item Began exploring the pipelines of their own teams.
    \item Found that his pipelines are really long. Then realized that it is because his pipelines are ensemble models.
    \item Sorted the primitives by importance. Identified that "CAST TO TYPE" correlates to worse scores. He said that this makes sense, because the dataset is textual, and this primitive is casting the string to a hash value. Therefore, this means that the hash is a bad feature for the problem.
    \item Identified that XGBoost GBTree primitive corresponds to the best pipelines.
    \item Using the graph comparison tool, he selected all pipelines from a system, and identified that they were using a template, only changing the classifier. (see figure x)
    \item Said that the system is useful to reverse engineer TA2 systems. His words: "Actually, with this tool we can infer what strategies people are doing with searches. (25:40)". "This tool is really nice to do reverse engineering."
    \item Looked at the top three performing pipelines. They were generated by the same system, and had the exact same primitives and graph structure. He thought it was interesting that the only thing this AutoML system was doing in this problem was tuning hyperparameters.
    \item He would like to query substructures in his ensemble models. I want to see if this smaller pipeline is being used  in the larger pipeline.
    \item Was interested in other team's pipelines, which used the same primitives and the same graph structure, but only changed hyperparameters
    \item His AutoML system used ensemble models. Therefore, he was interested in comparing his pipelines using the pipeline comparison tool and checking if there were repeated structures on his graphs.
    \item Found combination of primitives (check recording). Going to take note and add it to his AutoML rules. (generate templates based on his discovery)
    \item Was interested in the templates used by other teams.
\end{itemize}

Brandon (D4)
\begin{itemize}
    \item First thing i'm looking at are scores. How good are we at solving this problem. This is harder than some problems, F1 scores are close to .5. 
    \item What are the primitives involved in the produced pipelines? 
    \item Top three pipelines are nearly identical and have very similar scores. Identified primitives commonly used across pipelines that do not change the scores. Inputer does not change the scores.  Hypothesis:  There are not missing data in this dataset. If we wanted to simplify this pipeline, we could remove the primitives that do not affect the score (and are shared).
    \item He was curious what makes a pipeline bad in this dataset. He found that the "Random Classifier" produces bad scores, and noticed that it was used as a baseline score.
    \item Checked the time of pipelines and  identified that the best pipelines were also the fastest. Why is this pipeline so slow? Switched to the time view and used the primitive contribution to identify what primitives are really slow. He found that the general relational dataset makes the primitive slow. If I removed this primitive, I would get a faster pipeline. 
    \item In order to improve the results of pipelines, he wanted to compare his pipelines with the top scoring pipelines. I am using decision trees, and they are using gradient boosting. Gradient boosting is slightly more powerful, so if I substituted the decision tree by gradient boosting I would get better scores. It is almost a drop and replace operation to improve my scores in my pipeline search.
    \item He noticed that his pipelines are not setting many hyperparameters, instead using the default hyperparameters  from SKlearn. "In preprocessing, I should probably remove unnecessary primitives, and focus more of my AutoML search doing hyperparameter tuning."
    \item Teams are using a lot of pipeline templates. Do I need denormalize? Do I need this dataset reader (I only have one table)? It seems these things are included in some pipelines because they are part of the template, and not because they are useful.
\end{itemize}

Balazs (D3)
\begin{itemize}
    \item Identified that the best pipelines used random forest, but they had different scores. Looked at the hyperparameters of his pipelines and found many different values for random forest.
    \item He identified pipelines with ensemble random forest + gradient boosting. He said "It didn't help the pipeline, but it was an interesting idea."
    \item He identified a couple of outlier pipelines, with much higher Mean Squared Error values. He used the Edit operation to remove those pipelines from the analysis.
    \item He sorted the primitives by type and then spent some time analysing the different preprocessing primitives. One hot encoder does not help or hurt. The imputer in this case makes a big difference in scores (improves). 
    \item identified pipelines with different hyperparameters. "Ok, so in this case they used CNN with a bunch of different hyperparameters".
\end{itemize}

Sasawati (D1)

\begin{itemize}
    \item She prioritized scores in her analysis. She liked that the pipelines were numbered <team>: <number>, because she could compare the top pipelines from each team more easily.
    \item She identified that the best two pipelines have the same structure and graph, but use different hyperparameters. 
    \item Suggestion: vertical flow chart / graph
    \item What primitives they are using?
    \item What hyperparameters are they using? (used the extended table view)
    \item Identified outliers in the mean square error. Edit -> Removed selected pipelines. 
    \item "Being able to look at all pipelines together gives a very comprehensive picture of the data. "
    \item She noted that the best pipelines use XGBoost and explored the hyperparameter space of the best performing AutoML system. She mentioned she would incorporate more this primitive in their pipelines.
    \item In the past, what I have been doing is looking at the leaderboard. HOwever, it does not give us a detailed information about the pipelines. The results are not very user friendly. 
    \item She wanted to have a version of the system on the web.
\end{itemize}

\subsubsection{Evaluators Interview}

Shelly (E1)

\begin{itemize}
    \item She found out that pipelines were not linear, but DAGs. "I'm really blown away that pipelines are not linear. Because in the leaderboard they are shown as a list."
    \item Likes to sort pipelines by source and primitives by type. Tells us what kind of primitives different teams are using. The best scoring pipelines are always using the same types of primitives "Operators"
    \item At first we were only looking at scores and time. But now we are looking at: Are the teams solving the problems correctly? Are they using the correct primitives? Furthermore, are they solving the problems differently? Are they using a primitive that are giving them an advantage? How is the winning pipeline winning?
    \item Evaluators create pipelines by hand in order to try to beat the other systems. She would imagine using this system to find good configurations that would make the scores better. 
    \item They are interested in looking at the best pipelines for each team, and thinking about how they compare.
\end{itemize}

Swaroop Vattam (E2)

\begin{itemize}
    \item Dataset: carpool %LL1_726_TIDY_GPS_carpool_bus_service_rating_prediction_problem_TRAIN
    \item similar top scores
    \item Looked at the top scoring pipeline: used some type of scaling, text encoder (not sure why).
    \item I wonder why it's using a text encoder, there are not text features in this data.
    \item this makes sense to me. 
    \item Found that robust scaler is correlated with high scoring pipelines
    \item Found that the passive aggressive classifier is correlated with low scores.
    \item Found combination of primitives that could possibly result in a good performing pipeline: Robust scaler + Select FWE Feature extractor (15:20) and gradient boosting, I should be able to get a pretty good pipeline.
    \item Explained that this is not a causal relationship
    \item Used the combinatorial analysis to find that GradienT boosting and Mean Inputation correspond to better pipelines
    \item Investigated the hyperparameters of gradient boosting. Compared the hyperparameters of the top scoring pipeline against the others.
    \item For random forest, the default value of warm start is false. The pipeline that set it to true got a lower score. That makes sense, because the correct value should be false. 22:00
    \item compared the first pipeline with the second using graph diff. 
    \item Sorted pipelines by source. Compared strategies from multiple autoML.
    \item Compared pipelines across multiple datasets. Does CMU produces different pipelines for different classification problems? 
    \item Removed outliers
    \item For another problem, saw that few pipelines were using ARIMA, but said that this was the correct way to solve this problem. (sunspots + sunspots monthly)
    \item Looked at the UCB pipeline: Why is their pipeline looking so generic? Extra trees, construct predictions.
\end{itemize}

==> text/unused.tex <==

\subsubsection{AutoML Developer Insights}

Before they started the investigation, two developers had to remove outliers from their datasets. D1 and D3 selected datasets with a Mean Squared Error evaluation metric, which is unbounded in the positive real numbers. The two selected datasets, Auto MPG \cite{dua2017uci} and Sunspots \cite{sidc2019sunspots}, had pipelines with error metrics above $100,000.0$, which made the error metric scales difficult to read. In both datasets, the data scientists looked at the Primitive Contribution View and noted that a problem with the ``SGD'' primitive was responsible for these high errors.  Therefore, they used \systemname subset menu to remove these pipelines from the analysis.

Developers started the exploration by looking at the pipelines produced by their own systems and comparing how well they performed against the other AutoML tools. None of the interviewed developers had top scoring pipelines in the datasets that they chose to analyse. They used the Pipeline Matrix view to identify primitives used by the top scoring pipelines that their own systems were not using. For example, D4 inspected a classification dataset and  found that while a gradient boosting algorithm was used in the top scoring pipelines, his system was using decision trees. The Primitive Contribution view confirmed his hypothesis that the use of gradient boosting  was indeed  correlated with high scores. D4 then used the Pipeline Comparison View to check whether there were any other differences between his and the best performing pipelines, but found that they were mostly equal. He mentioned that he could use this insight to drop and replace primitives in his AutoML search space. D1, D2 and D3 had similar findings in their pipeline investigations.

Data scientists also used \systemname to identify primitives that should be removed from their pipelines. D2 investigated the primitives using the Primitive Contribution view, and found that pipelines containing the ``Cast to Type'' primitive resulted in lower F1 scores. He inspected the hyperparameters of this primitive and noted that string features were being converted to float values (hashes). Therefore, he concluded that string hashes were bad features for this classification problem, and the ``Cast to Type'' primitive should be removed from those pipelines. D3's dataset consisted of a numerical matrix with no missing values. However, he noticed that some of his pipelines used the primitives ``One hot encoder'' (which transforms categorical features in numerical features) and ``Inputer'' (which inputs missing values in matrices). The primitive contribution view showed him that these primitives had no correlation with the scores, confirming his hypothesis that they did not help his pipelines. Therefore, D3 decided to add rules to his AutoML system so that unnecessary primitives were not added. Similarly, D4 noted that some AutoML systems were using templates and just changing the classification algorithm, which resulted in pipelines with unnecessary primitives. D4 also found that for his dataset, ``Imputer'' primitives were unnecessary.

D4 wanted to check the running times of the pipelines. In particular, he was interested in knowing whether the best pipelines took longer to run. First he sorted the pipelines by score. Then, he switched the displayed metric to ``Time'' and noticed that, contrary to his original hypothesis, the best pipelines were also the fastest. He looked at the Primitive Contribution View in order to find what primitives were responsible for the longer running times, and identified that the ``General Relational Dataset'' primitive was most likely the culprit. He concluded that if he removed this primitive, he would get a faster pipeline. 

D2's AutoML system is able to create ensemble pipelines (pipelines where multiple ML algorithms work together to form a single output). D2 noticed that his pipelines were using more primitives then the other teams, and hypothesized that this was because of the ensemble nature of his AutoML. He visualized the pipeline graphs of his pipelines and confirmed that the output of multiple classifiers were being combined in order to generate the final output predictions. D3 found smaller ensemble models on his pipelines, consisting of both random forests and gradient boosting. However, he noted that these models did not perform better than simpler models, and decided to drop the random forest from similar cases in the future. 

The data scientists also spent some time exploring the primitive hyperparameters, especially those of the best scoring pipelines. D1 noticed that the top five pipelines for her chosen dataset belonged to the same AutoML system, and were nearly identical: they used the same primitives and had the same pipeline graphs. She explored the hyperparameters of these pipelines using the  one-hot-encoded hyperparameter view, and found that although they had the same graph structure, they were using different hyperparameters. In particular, she noted that the AutoML system focused it's hyperparameter tuning stage on the ``Gradient Boosting'' primitive, tuning five of its values.

\subsubsection{AutoML Evaluator Insights}

While developers used \systemname to find points of improvement for their algorithms, evaluators focused on comparing the different AutoML systems. The first comparison E1 did was using the pipeline scores. She grouped pipelines by source and noticed the difference in scores among the top pipelines from each AutoML system. The top two AutoML systems had pipelines with F1 Scores of 0.78 and 0.70, which she mentioned were very close. The other systems produced pipelines with much lower scores, below 0.25. E2 also sorted pipelines by source, and noticed that most AutoML had at least one pipeline with an F1 Score of 0.6, with the exception of two AutoML systems (max scores 0.56 and 0.21).

E1 told us that she would like to use the tool to check whether teams were using the different primitives to solve a particular ML problem. She grouped primitives by type in the matrix representation, noted that the top AutoML algorithm was using ``LSTM CNN'' in most of it's pipelines, and focused on tuning the hyperparameters of this primitive. She discovered that the second best AutoML system had more diverse solutions, using three different classifiers: ``K Nearest Neighbors'', ``Random Forrest'' and ``SVC''. The lower scoring pipelines had even more diverse primitives.

E2 looked at the Primitive Contribution View and found primitives correlated with high scores. Using this view, he started to formulate hypothesis about the pipelines, for example: ``If I create a new pipeline that contains a Robust Scaler, Select FWE feature extractor and Gradient Boosting, I should be able to have a pretty good pipeline''. E2 understood that the Primitive Contribution View does not show a causal relationship, but he was excited to test the hypothesis. E2 also used the Combinatorial Primitive Contribution table to see groups of primitives that worked well together: he found that together, ``Gradient Boosting" and ``Denormalize'' were correlated with high scores.

Finally, E1 also said they were evaluating whether the pipelines solved the problem correctly, using the right primitives for the task at hand. For example, similarly to D3 and D4, she noticed that some teams were using the primitives ``Inputer'' and ``One Hot Encoder'' unnecessarily. E2 made a similar observation: he saw that some pipelines used ``Text Encoder'' primitive, but was not sure whether it was needed. He investigated the training data and found that it indeed contained one textual column, so the use of ``Text Encoder'' made sense. 

E2 was also interested in looking at the primitive hyperparameters, in order to check for correctness. For example, he expanded the Pipeline Matrix with the One Hot Encoded representation of the Random Forest hyperparameters. He noticed that one AutoML system always set the ``warm start'' parameter to ``true''. However, he said that in this case, the correct value should be false. 










\section{Primitive contribution}

Machine Learning explanation methods such as LIME \cite{ribeiro} and SHAP \cite{shap} produce weights that explain the behavior of a classifier by creating new points in the neighborhood of a sample and investigating the classifier output on the new points. Intuitively, the same formulation could be used to estimate the primitive contribution to pipeline scores, as the inputs and outputs are very similar. We would like to predict how well a pipeline will perform on a dataset and task, and also explain which primitives contributed the most for this score. However, generating new pipelines is not a trivial task, given that not only we need to select a group of primitives that have compatible inputs and outputs, but also we have to create the connections between these primitives. Such a task needs to be completed by an AutoML system, and is not generalizable across systems. Furthermore, running each new pipeline to evaluate its scores is not computationally tractable.

Given the complexity of creating and running new pipelines, model explanation techniques are not appropriate for computing the scores of 

Let $M$ be the indicator matrix, where $m_{ij}$ is $1$ if pipeline $i$ contains the primitive $j$ and $0$ otherwise. Let $U_j$ be the set containing the indices of the rows of M that uses primitive $j$, and $\bar{U}_j$ be set containing the indices of the rows of M that does not use primitive $j$.

$$
U_j = \{i | M_{ij} = 1\} 
$$

$$
\bar{U}_j = \{i | M_{ij} = 0\} 
$$

We define the primitive contribution $\phi$ as 

$$
\phi(F_i) = \frac{\sum\limits_{k \in U_j} s_k}{|U_j|} -  
\frac{\sum\limits_{l \in \bar{U}_j} s_l}{|\bar{U}_j|}
$$


\section{D3M Data and Pipeline}

Pipelines are represented as JSON or YAML serialized objects in memory . A pipeline consists of: (1) Pipeline metadata, (2) specification of inputs and outputs, and (3) definition of pipeline steps. The first one contains mostly non-essential information like name and description, the only required metadata is the pipeline’s universally unique identifier (UUID) \cite{uuid_2005}. The second one contains a description of inputs and outputs that the pipeline has, optionally it can provide human-friendly names for them. Finally, the last one, defines the logic of the pipeline. They are specified in order and each step defines its inputs and outputs and how step’s inputs are connected. There are three types of steps: (a) Primitive steps, which represent execution of a primitive. (b) Sub-pipeline step, which represents execution of another pipeline as a step, and (b) Placeholder step, which represents partially defined pipelines (\textit{pipeline templates}). Note that primitives are basic building blocks of pipelines. They can be either defined as regular function with pre-defined logic, or can learn it given example inputs and outputs (\textit{learnable functions}). \todo{Say that pipelines are generic data structures, but for our use case consists in <simplified data>}

With recent advances in Automatic Machine Learning (AutoML), it is now possible to create end-to-end machine learning pipelines that solve complex real world problems without human intervention  \cite{hutter_automated_2019, drori_alphad3m:_2018}. Commercial \cite{google_cloud_2020, mljar_machine_2020, ibm_watson_2020} and open-source \cite{drori_alphad3m:_2018, olson_tpot_2019, feurer_auto-sklearn_2019, santos_visus_2019} AutoML systems use different approaches to explore a large model search space and optimize the model hyperparameters, but due to their black box nature, it is hard for data scientists to evaluate, compare and improve them \cite{wang_atmseer:_2019}. Such systems produce a large number of machine learning pipelines, and currently there are repositories with thousands of AutoML pipelines available for download \cite{D3M2020metalearning}. By analyzing these pipeline collections, we have the opportunity to better understand how these systems work and obtain insights that can be used to improve them. However, this is challenging due both to the large number of pipelines and their complex structure.

